Is the Elephant Flying? Resolving Ambiguities in Text-to-Image Generative Models

Natural language often contains ambiguities that can lead to misinterpretation and miscommunication. While humans can handle ambiguities effectively by asking clarifying questions and/or relying on contextual cues and common-sense knowledge, resolving ambiguities can be notoriously hard for machines. In this work, we study ambiguities that arise in text-to-image generative models. We curate a benchmark dataset covering different types of ambiguities that occur in these systems. We then propose a framework to mitigate ambiguities in the prompts given to the systems by soliciting clarifications from the user. Through automatic and human evaluations, we show the effectiveness of our framework in generating more faithful images aligned with human intention in the presence of ambiguities.

==> sections/2-intro.tex <==
\section{Introduction}
Natural conversation inherently contains ambiguities due to potentially multiple interpretations of the same utterance. A few categories of ambiguities are: (i) \textit{syntactic} ambiguity, (e.g., ``an elephant and a bird flying” — is the elephant flying?), (ii) \textit{semantic} ambiguity, (e.g., ``show me picture of cricket” — is cricket referring to an insect or a game?), and (iii) ambiguity due to \textit{underspecification} (e.g., ``doctor talking to a nurse” — is the doctor/nurse male or female?). 

The ambiguities associated with underspecification can lead to development of different types of biases, such as gender bias. This is due to the fact that underspecification can result the models or humans encountering them to inject their own stereotypes or biases to fill in the gap that was left out in the original prompt due to underspecification. This suggests that language ambiguities can lead to biased outcomes with possible implications for fairness of the underlying models. Using ambiguous prompts in language modeling can also lead to issues such as misinformation and development of fallacies, which can result in poor user satisfaction. This is due to the fact that a wrong interpretation of an ambiguous prompt can lead into development of falsified hypothesis that can result in development of fallacies as well as misinformation. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\linewidth,trim=2.5cm 0.3cm 16cm 0cm,clip=true]{images/intro-pic.pdf}
    \vspace{-.07in}
    \caption{Examples of ambiguous prompts and corresponding generated images. The icon between the images depicts alternative interpretations. The images corresponding to first two prompts are generated by DALL-E Mega~\cite{Dayma_DALL}, and images corresponding to last two prompts are generated by OpenAI's DALL-E~\cite{ramesh2022hierarchical} models.}
    \label{fig:motivation}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth,trim=1cm 8cm 1.5cm 0.2cm,clip=true]{images/framework.pdf}
    \vspace{-.07in}
    \caption{Our proposed disambiguation framework. The initial ambiguous prompt is disambiguated by either (1) the language model generating clarifying question which will be resolved through human provided answers, or (2) the language model generating different possible visual setups and human-agent choosing the desired setup. The final disambiguated prompt will later be provided to the downstream text-to-image generative model.}
    \label{fig:framework}
\end{figure*}

With the growing popularity of text-to-image generative models, in this paper, we study the effect of ambiguity in these  models~\cite{ramesh2021zero,ramesh2022hierarchical,saharia2022photorealistic,yu2022scaling}. We also propose a framework for mitigating ambiguities existing in prompts. We choose this setting to study ambiguity as visual scenes provide readily human-interpretable alternative understandings of text, thus helping in evaluating ambiguities as well as mitigation strategies. Figure~\ref{fig:motivation} illustrates some sample prompts and corresponding outputs from the state-of-the-art text-to-image model, DALL-E. We observe that ambiguity in the prompts confuses the model resulting in a varied set of generated images. 

Humans tend to resolve ambiguities by asking clarifying questions, relying on other forms of modalities (such as vision), using contextual signals, and leveraging commonsense and/or an external source of knowledge~\cite{ACHIMOVA2022104862}. Inspired by  this observation, we propose a new framework (Figure~\ref{fig:framework}) in which we incorporate a language model-based {\em prompt disambiguation filter} on top of the text-to-image generative models. This filter is capable of either asking clarifying questions or generating different possible setups which would later be resolved through human interactions. Ultimately, the disambiguation filter helps the text-to-image model to identify a single visual setup for image generation. 


To better understand the weaknesses of current text-to-image generative models, and to evaluate the effectiveness of our proposed mitigation framework, we  curate a benchmark dataset consisting of ambiguous prompts covering different types of ambiguities that are especially relevant to text-to-image models. We also propose new automatic evaluation procedures to evaluate faithfulness of generations in text-to-image generative models and compare it with human evaluations. We perform various automatic as well as human evaluation experiments to further validate our claims. 

Overall, we make the following contributions:
\begin{enumerate}
\item We introduce a benchmark dataset containing ambiguous prompts along with different visual setups (Section~\ref{sec:bench}).
\item We propose new automatic evaluation procedures to evaluate ambiguity resolution in text-to-image models (Section~\ref{sec:eval_method}).
\item We propose a disambiguation framework which can be applied on any text-to-image model. We use our benchmark dataset and the metrics to evaluate multiple variations of DALL-E as well as our disambiguation framework (Section~\ref{sec:framework}).
\end{enumerate}






==> sections/2-intro__archived_.tex <==
\section{Introduction}
Natural conversation is expected to contain ambiguous mentions and references. Humans tend to resolve ambiguities by asking the person they are interacting with to clarify, rely on other forms of modalities (such as vision or taste), or in some cases use commonsense and/or an external source of knowledge~\cite{ACHIMOVA2022104862}. While humans are naturally good in resolving ambiguities in most cases, Artificial Intelligent (AI) systems are not~\cite{JACKSON2020209}. This is in part due to the fact that many AI applications are stand-alone and are limited in doing commonsense reasoning. For instance, a stand-alone vision application does not utilize capabilities of a language model to improve itself. Although with the rise of multi-modal models researchers have tried to improve these systems by leveraging synergies between different modalities, these models still lack human-level capabilities mostly due to the fact that they do not fully mimic human behavior.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\linewidth,trim=2.5cm 0.3cm 16cm 0cm,clip=true]{images/intro-pic.pdf}
    \vspace{-.07in}
    \caption{Examples of ambiguous prompts and corresponding generated images from DALL-E Mega~\cite{Dayma_DALL} and OpenAI's DALL-E~\cite{ramesh2022hierarchical}. The images corresponding to first two prompts are generated by DALL-E Mega, and images corresponding to last two prompts are generated by OpenAI's DALL-E models.}
    \label{fig:motivation}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth,trim=1cm 8cm 1.5cm 0.2cm,clip=true]{images/framework.pdf}
    \vspace{-.07in}
    \caption{Our proposed disambiguation framework. The initial ambiguous prompt is disambiguated by either the language model generating clarifying question which will be resolved through human provided answers, or the language model generating different possible visual setups and human-agent choosing the desired setup. The final disambiguated prompt will later be provided to the downstream text-to-image generative model.}
    \label{fig:framework}
\end{figure*}

Recently, text-to-image generative models, which integrate both capabilities of a language and visual models, got significant attention~\cite{ramesh2021zero,ramesh2022hierarchical,saharia2022photorealistic,yu2022scaling}. However, these models are also far from resolving ambiguities as humans do despite the fact that they incorporate both vision and language models jointly. For instance, for given ambiguous prompts shown in Figure~\ref{fig:motivation}, it is not clear which image should be generated by these text-to-image generative models. This is due to the fact that these models do not mimic human behavior upon encountering ambiguous prompts. In such situations, given an ambiguous prompt, a human would either ask for clarifying questions to resolve ambiguities or will reason some options and will try to pick the best option based on an external signal. 

Inspired by such human behavior as well as the idea of incorporating different models together to build an improved AI system, we propose a new framework in which we incorporate a language model on top of  text-to-image generative models that are capable of reasoning similar to humans in either asking for clarifying questions or generating different possible setups which would later be resolved through human interactions. This serves as a prompt disambiguation filter that sits on top of the text-to-image model. 

To evaluate the effectiveness of our proposed framework, as well as showcasing the weaknesses of current text-to-image generative models, we also curate a benchmark dataset consisting of ambiguous prompts covering different types of ambiguities that are relevant to text-to-image models. In addition, we propose new automatic evaluation procedures to evaluate faithfulness of generations in text-to-image generative models and compare it with human evaluations. We perform various automatic as well as human evaluation experiments to further validate our claims. 

We highlight the importance of resolving ambiguities as well as our work by pointing out the issues that arise in the existence of ambiguous prompts. Ambiguous prompts can result in misinformation, development of fallacies, poor user satisfaction, and biased outcomes-- in cases where there is not enough information about an identify of an individual with implications on fairness. In this work, we frame the development of bias as a form of ambiguity that the system is not able to resolve. These ambiguities can result in the system making overgeneralized assumptions about the identity of an individual~\cite{mehrabi-etal-2021-lawyers}.




